Holographic Beam Measurements of the Canadian Hydrogen Intensity Mapping Experiment (CHIME)

We present the first results of the holographic beam mapping program for the Canadian Hydrogen Intensity Mapping Experiment (CHIME). We describe the implementation of the holographic technique as adapted for CHIME, and introduce the processing pipeline which prepares the raw holographic timestreams for analysis of beam features. We use data from six bright sources across the full 400-800\,MHz observing band of CHIME to provide measurements of the co-polar and cross-polar beam response of CHIME in both amplitude and phase for the 1024 dual-polarized feeds instrumented on CHIME. In addition, we present comparisons with independent probes of the CHIME beam which indicate the presence of polarized beam leakage in CHIME. Holographic measurements of the CHIME beam have already been applied in science with CHIME, e.g. in estimating detection significance of far sidelobe FRBs, and in validating the beam models used for CHIME's first detections of \tcm emission (in cross-correlation with measurements of large-scale structure from galaxy surveys and the Lyman-$\alpha$ forest). Measurements presented in this paper, and future holographic results, will provide a unique data set to characterize the CHIME beam and improve the experiment's prospects for a detection of BAO.

==> appendices.tex <==
\appendix



==> holography.tex <==
\section{Description of the holographic technique}
\label{sec:holo_description} 
Holographic measurements of a radio dish have a long history in radio astronomy, primarily as a means of measuring the surface figure of a telescope dish and comparing it to specifications. For a theoretical overview of the technique, see e.g. \citep{1966holotheory, holographyscottryle}; for some examples of applications of the technique to more traditional radio telescopes, see e.g. \citep{holography30m, holographyeffelsberg100m, holographyyebes40m} and the historical account from \citep{baarsholohistory}.  Using holography to map the far-field beam of a cylindrical telescope was first demonstrated on the CHIME pathfinder array \citep{bergerholo}.

Holographic measurements consist of two radio dishes: a `dish under test' whose beam is being characterized and a reference dish. For the holographic measurements of CHIME, the CHIME inputs are under test, and the co-located steerable 26\,m John A. Galt telescope is the reference dish (see \citealt{galt_spie_proc} for details on the Galt telescope, as instrumented for holography with CHIME). The Galt telescope tracks a source as it transits through the CHIME beam, and the signals from CHIME and the Galt telescope are correlated in the CHIME correlator. This correlation measures only what is common between the Galt beam and the larger CHIME primary beam, reducing the confusion noise on a given point source. The resulting interferometric data set provides a measurement of the amplitude and phase of the CHIME far-field beam pattern in both co-polarization and cross-polarization, for each of the 1024 dual-polarized CHIME feeds at all 1024 frequencies. This far-field pattern can be transformed to provide a map of the aperture (as would be done for most holography applications). Because the confusion noise is reduced, this technique provides high signal-to-noise measurements of the CHIME primary beam along the East-West trajectory at the declination of the transiting source. This provides an assessment of sidelobe power which is broadly useful for CHIME science; for example, this sidelobe information was used in \citep{farsidelobefrbs} to obtain signal-to-noise ratios for detections of far-sidelobe FRBs.  After applying an overall calibration per observation (see Section \ref{sec:stacking}), the holographic system is sufficiently stable that multiple observations of a single source can be co-added to improve signal-to-noise. Even with co-adding, only about $\sim$20 sources are bright enough to warrant targeting via the holographic technique, thus it cannot be used to fill the North-South beam. In spite of its sparse declination coverage, holography has excellent synergy with independent probes of the CHIME beam, as the polarization, phase, and per-feed variation of the beam are hard to measure without holography. 
%\jm{It might be nice to remind the reader here of why holography is useful, even though it can't be used to fill the NS beam. E.g. "Despite the sparsity in declination coverage, holography provides valuable phase and polarization information that is otherwise hard to measure, and hence it has excellent synergy with other beam measurements."}. 
\subsection{General formalism}
\label{sec:holo_tech}
%As such, the technique utilizes two telescopes: the dish under test, and a reference dish. Both telescopes observe the same calibrator in the far field and their responses are correlated. For holography with CHIME, the ``dish under test" is each of the 1024 dual-polarisation feeds individually, and the reference dish is the co-located Galt 26\,m telescope. 
Holography is an interferometric measurement of the complex (i.e.\ amplitude and phase) far-field response of a radio telescope, obtained by correlating the signals measured by the antenna under-test and the reference dish while observing a common calibrator. In general, the polarised response of the $i$-th CHIME feed (under-test), as a function of sidereal time $\phi$ and frequency $\nu$, to the sky can be written as follows:
%
\begin{equation}
    F^a_i(\phi, \nu) = \int d^2\mathbf{\hat{n}} J^{ap}_i(\mathbf{\hat{n}}; \nu)\epsilon_p(\mathbf{\hat{n}}; \phi, \nu)e^{2\pi i \mathbf{\hat{n}}\cdot\mathbf{u}_i} 
\end{equation}
%
%\tpm{Maybe nitpicking here, but if the coordinate $\mathbf{n}$ is fixed to the telescope frame and it's the sky that is varying with $\phi$, then $J$ is independent of $\phi$, no? Or is it allowed to drift with temperature or something?}
where $J^{ap}_i$ is the (direction-dependent) Jones matrix of the CHIME feed, including the beam response, $\epsilon_{p}$ is the vector electromagnetic field density defined on the celestial sphere and incident on the feed,  $\mathbf{\hat{n}}$ denotes a position on the sky in the coordinate frame of the telescope, and $\mathbf{u}_i$ is the position vector (in units of wavelength) of the feed measured from an arbitrary origin point (when we take the cross-correlation with the Galt response, the origin point will be irrelevant). One can write an analogous expression for the response of the (reference) Galt telescope, 
\begin{equation}
    F^b_{26}(\nu) = \int d^2\mathbf{\hat{n}} J^{bq}_{26}(\mathbf{\hat{n}}_{26}\left[\mathbf{\hat{n}};\phi\right]; \nu)\epsilon_q(\mathbf{\hat{n}}; \nu)e^{2\pi i \mathbf{\hat{n}}\cdot\mathbf{u}_{26}} 
\end{equation}
where $J^{bq}_{26}$ is the Jones matrix of the Galt telescope and $\mathbf{\hat{n}}_{26}\left[\mathbf{\hat{n}}; \phi\right]$ transforms the coordinate $\mathbf{\hat{n}}$ into a coordinate measured with respect to the boresight of the Galt telescope at time $\phi$. $\mathbf{u}_{26}$ is the position vector (in units of wavelength) of the Galt telescope from the same (arbitrary) origin point.

%\simon{
%In Eq. (1), $\mathbf{\hat{n}}$ is defined in the CHIME telescope frame. Eq.\ (2) uses the same $\mathbf{\hat{n}}$ everywhere, but I'd expect the $G^{bq}_{26}$ in Eq.\ (2) to only depend on the difference between a given sky location and the instantaneous direction of the Galt boresight. I think the minimal way to resolve this would be to rewrite Eq.\ (2) as something like 
%\begin{equation*}
%    F^b_{26}(\nu) = \int d^2\mathbf{\hat{n}} 
%    G^{bq}_{26}(\mathbf{\hat{n}}_{26}[ \mathbf{\hat{n}}; \phi ]; \nu)
%    \epsilon_q(\mathbf{\hat{n}}; \nu)e^{2\pi i \mathbf{\hat{n}}\cdot\mathbf{u}_{26}} \ ,
%\end{equation*}
%where $\mathbf{\hat{n}}_{26}[ \mathbf{\hat{n}}; \phi ]$ tranforms $\mathbf{\hat{n}}$ into angular coordinates that are defined with respect to the Galt boresight at a given sidereal time.
%
%On the other hand, this would require a few changes to later equations. Am I misunderstanding the meaning of $G^{bq}_{26}$?
%}

The indices $a (b), p (q)$ distinguish the states of chosen instrumental and on-sky polarization bases. For CHIME, we use a linear polarization basis $a \in \{X, Y\}$, with $X$ polarization orthogonal to the CHIME cylinder axis and $Y$ parallel to it. For the Galt telescope, the polarization basis indexed by $b$ is not fixed relative to CHIME due to the motion of the dish over the course of an observation, however the feed is aligned such that its polarization axes align with that of CHIME when the telescope is pointed to the meridian. The indices $p, q$ belong to an on-sky polarization basis, and the Jones matrices $J_{i, 26}$ then define a mapping between on-sky polarization and the polarization measured by the instruments. 
%\tpm{Maybe for completeness, define $\mathbf{n}$, the position on the fixed sky. Consider using $\mathbf{\hat{n}}$. Also, and this may be unnecessary, but isn't it true that the sky polarisation index $b$ refers to a different basis than $X, Y$ (and $J$ encodes the projection between the two)?} \arcomment{Yeah, this is true. I have reworded the end of the preceding paragraph to emphasize that the choice of a linear polarisation basis is made for the instrument frame and that J maps from the sky-frame to the instrument-frame.}
%\lbn{in our case, the linear polarization states XX, XY, YX, and YY \arcomment{Changed}}. 
%\jm{Is it worth breifly stating the polarization convention for Galt here since the same was done for CHIME in the previous paragraph? Also I don't mean to nitpick, but starting in equation 2 and onward, I think the frequency dependence was omitted from some quantities without saying that this would be dropped going forward.} 

In CHIME holography, we form the cross-correlation of the $i$-th CHIME feed and the Galt feed. In general this cross-correlation takes the form:
\begin{align}
\nonumber
    V^{ab}_{i, 26}(\phi, \nu) &\equiv \left<F^{a}_iF^{\dagger b}_{26}\right> \\
    &= \int d^2\mathbf{\hat{n}}\int d^2\mathbf{\hat{n}}'J_i^{ap}\left<\epsilon_p\epsilon^*_q\right>J_{26}^{*qb}e^{2\pi i \left(\mathbf{\hat{n}'}\cdot\mathbf
    {u}_{i}- \mathbf{\hat{n}}\cdot\mathbf{u}_{26}\right)}
\end{align}
%\tpm{With the convention you defined above, the sign in the exponent here is wrong, and you should have $\epsilon_q^*$.}
%\lbn{alignment looks wierd ... might recommend right aligned?\arcomment{Fixed}}
%\tpm{(here and elsewhere, formatting would look better if you didn't have a new line between the equation and text.)} \ac{(as Tristan mentioned, you need to change $\epsilon_q^*$ in the following lines too )}\arcomment{Fixed.} 
%\simon{There's some inconsistency in the upper index ordering of $J$ and $G$. Eq.\ 1, $J_i^{ab}$ has the first index $a$ as a CHIME pol and $b$ as an on-sky pol, while in Eq.\ 3, $J_i^{*qa}$ has the first index $q$ as an on-sky pol and the second index $a$ as a CHIME pol. The same flip happens for $G$ from Eq.\ 2 to Eq.\ 3. Eq.\ 5 implies that the indices of $J$ should be (on-sky pol, CHIME pol) and the $G$ indices should also be (on-sky pol, CHIME pol). I think the natural interpretation of your ``*" superscript is that the quantity is complex-conjugated but the index order is {\em not} swapped, since ``$\dagger$" is reserved for a Hermitian conjugate.}
where the product $\left<\epsilon_p\epsilon^*_q\right>$ is the coherency matrix of the sky signal. 

In practice, the experimental setup allows us to simplify this expression considerably. First, we assume that the electric fields from the astronomical source are spatially incoherent; i.e., the coherency term will introduce a factor $\delta(\mathbf{\hat{n}} - \mathbf{\hat{n}}')$ which eliminates one of the integrals. Second, we note that we perform holographic measurements of \textit{point-source} calibrators transiting over CHIME in tracks of constant declination. To CHIME, the source has a time-dependent position $\mathbf{\hat{n}}_\text{src}(\phi)$, while the Galt telescope tracks the source throughout the observation. This is expressed as a $\delta$-function spatial dependence in the sky coherency term, i.e.\ we will write $\left<\epsilon_p\epsilon^*_q\right> \equiv T^\text{src}_{pq}\delta(\mathbf{\hat{n}} - \mathbf{\hat{n}}_\text{src})$, where $T^\text{src}_{pq}$ is a matrix describing the polarized emission of the point source.  The $\delta$-function collapses the remaining integral to the direction of the calibrator, leaving us with 
%\tpm{I think the coordinates may be getting confused here. Is $\mathbf{n}$ meant to be a sidereal coordinate or a telescope coordinate? i.e. is $J$ or $\mathbf{n}$ a function of $\phi$. Then, strictly speaking shouldn't your equation with the $\delta$'s really be two steps? The electric field is uncorrelated spatially ($\delta(\mathbf{n} - \mathbf{n}')$) and then the Galt beam can be approximated as collapsing the intergral because it is compact compared to the CHIME beam ($\delta(\mathbf{n} - \mathbf{n}_\text{src})$).}
%\lbn{might recommend B -> T, since B is for beam a lot of times in related-looking equations\arcomment{Changed accordingly}}
\begin{align}
\label{eq:holo_vis_general}
   V^{ab}_{i, 26}(\phi, \nu) = 
 J^{ap}_i(\mathbf{\hat{n}}_\text{src}(\phi);  \nu)T^\text{src}_{pq}(\nu)J^{*qb}_{26}(\nu) \\ \times
 e^{2\pi i\mathbf{\hat{n}}_\text{src}(\phi)\cdot\mathbf{u}_{i, 26}} 
\end{align}
%\simon{Should $\mathbf{n}_\text{src}$ also be a function of $\phi$ in the exponent?}
where we have written $\mathbf{u}_{i, 26} = \mathbf{u}_i - \mathbf{u}_{26}$. We have dropped the direction-dependence of the 26\,m's Jones matrix because when we collapse the integrals to the location of the source, only the boresight response of the 26\,m remains. 
Combining the phase factor with the sky brightness factor $T^\text{src}_{pq}$, we can write the holographic response for all polarization products compactly in matrix form as: 
\begin{equation}
    \mathbf{V}_{i, 26}(\phi, \nu) = \mathbf{J}_i(\mathbf{\hat{n}}_\text{src}(\phi); \nu)\mathbf{T}_\text{src}(\nu)\mathbf{J}^\dagger_{26}(\nu) \ . 
\end{equation}
Given the Jones matrix of the Galt telescope and a suitable, well-known calibrator (i.e.\ a well-constrained $\mathbf{T}_\text{src}$), one could invert this expression to solve for the Jones matrix of CHIME feed $i$. However, as we  have ignored instrumental noise, this represents only a schematic illustration of the technique rather than a formal estimator for CHIME's Jones matrix. In practice, there are additional confounding factors beyond instrumental noise: among the most pressing is that the Jones matrix of the Galt telescope is difficult to calibrate independently, as its equatorial mount precludes typical polarimetric calibration through measurements of polarised sources over a range of parallactic angles. In the past (for a different receiver system and observing band), electromagnetic simulations have been used to compute the response of the Galt telescope to polarized emission (see \citealt{tomgalt}). For our purposes, however, a holography-based full-Jones matrix calibration of CHIME, which would include the effects of parallactic angle rotation and polarisation leakage / differential gain in the signal chain, is beyond the scope of this paper. Instead, we directly measure the direction-dependent products $\mathbf{V}_{i, 26}(\phi, \nu)$; in the case that $\mathbf{T}_\text{src}$ and $\mathbf{J}_{26}$ are diagonal, these products yield the CHIME $X$ and $Y$ beams up to an overall normalization. 

\subsection{Confusion noise} %[Alex]}
\label{sec:confusion_noise}


One of the limitations of CHIME-only techniques to measure the CHIME primary beam is the confusion noise associated with the instrument's large instantaneous field of view. Direct observations of calibrator sources quickly become confusion limited off-meridian. Solar measurements of the beam avoid this problem due to the brightness of the Sun, but these data are only available in the southern sky due to the limited declination range of the Sun. In holography, the effect of confusion is significantly reduced because the correlation between CHIME and the Galt telescope removes all confusing sources which are outside the Galt telescope's much smaller (compared to CHIME) beam. Here we outline a procedure to estimate the remaining confusion noise limit of the holography data. 

We proceed from Equation \ref{eq:holo_vis_general}, where we will drop the polarization indices, considering scalar quantities (i.e.\ in only Stokes I)  instead of the matrix quantities appearing in the fully polarized treatment (i.e.\ following the discussion at the end of Section \ref{sec:holo_tech}, we will replace Jones matrices $J_i, G_{26}$ with primary beam factors $A_i, A_{26}$). Then, a holographic visibility at a single frequency and sidereal time can be written schematically in the following way: 
\begin{equation}
    V_{26, i} = A_i(\mathbf{\hat{n}}_\text{src})A_{26}(\mathbf{\hat{n}}_{\text{src}})T_\text{src}(\mathbf{\hat{n}}_\text{src})e^{2\pi i(\mathbf{u}_i - \mathbf{u}_{26})\cdot\mathbf{\hat{n}}_\text{src}}
\end{equation}
%\ac{[will there be a $\mathbf{\mathbf{\hat{n}}_{src}}$ in eqn 4 and 5 in G term? which is saying the beam or matrix along source direction but not a function of $\mathbf{\phi}$]}
where $A_i$ is the primary beam response of CHIME feed $i$, $A_{26}$ is the primary beam of the Galt telescope and the other symbols are as defined in Section \ref{sec:holo_tech}.  %\tpm{there should only be one direction vector in this equation, and it might be useful to make clear that $\mathbf{n}(\phi)$ is confined to a 1-d track of constant declination.}
%During a holography observation, the Galt telescope tracks a bright point source across the sky, so that the sky brightness could be represented by a single delta function centered at $\mathbf{n_{\text{cal}}}$ with strength equal to the source brightness. 
%\simon{Although you say that this equation is schematic, it confuses me that the matrix nature of the quantities in this equation has suddenly disappeared. Some more explanation would be helpful}\arcomment{I added some extra verbiage to the preceding paragraph to try to be a little more explicit about what's going on here.}

To account for the confusing background of unresolved sources within the Galt beam, we now model the brightness temperature as a sum over sources (indexed by $a$ in the following equations) within the Galt beam (``FoV"). The visibility then reads 
\begin{equation}
    V_{26, i} = \sum_{a \in \text{FoV}} A_i(\mathbf{\hat{n}}_a)A_{26}({\mathbf{\hat{n}}_a})T(\mathbf{\hat{n}}_a)e^{2\pi i (\mathbf{u}_i - \mathbf{u}_{26 })\cdot\mathbf{\hat{n}}_a} + \text{src}
\end{equation}
where $+ \text{src}$ represents the contribution of a like term from the actual calibrator source; i.e., the proper holographic visibility we are attempting to measure. The $\mathbf{\hat{n}}_a$ are the sky positions of confusing sources which are near the telescope boresight, i.e., $\mathbf{\hat{n}}_a = \mathbf{\hat{n}} + \delta\mathbf{\hat{n}}_a$. 

As the CHIME-Galt baseline fringes rapidly, the geometric phases of the confusing sources are expected to decohere so that the average confusion bias over all sources is negligible. To estimate how the confusion noise may limit our measurement's signal-to-noise, we need to determine the overall confusion noise level. This can be obtained from the variance of the first term across sources:
\begin{align}
\nonumber
    \text{Var}[V_{26, i}]_\text{conf} = |A_i|^2 \sum_a\sum_bA^*_{26}(\mathbf{\hat{n}}_a)A_{26}(\mathbf{\hat{n}}_b)T(\mathbf{\hat{n}}_a)T(\mathbf{\mathbf{\hat{n}}}_b) \\
    \times \left<e^{2\pi i (\mathbf{u}_i - \mathbf{u}_{26})\cdot(\mathbf{\hat{n}}_a - \mathbf{\hat{n}}_b)}\right>
\end{align}
%\simon{Maybe displaying my ignorance, but: the variance is literally the square of the first term from the previous equation? There's no type of ensemble-averaging involved?} \arcomment{This equation is using the definition of variance $\text{Var}[X] = \left<(X - \Bar{X})^2\right>$, where the mean here across sources is argued to be zero because the holographic phase factor will decohere when summing over confusing sources.}
where the $A_i({\bf{n}})$ factor from the CHIME beam has been factored out under the assumption that the CHIME beam varies slowly on scales comparable to the beam width of the Galt telescope.
 As the interferometric phase will decohere for different sources, the ensemble average over the confusing phase term will be non-zero only for $\mathbf{\hat{n}}_a = \mathbf{\hat{n}}_b$, collapsing one of the sums, so that the noise variance reduces to
\begin{equation}
    \text{Var}[V_{26, i}]_\text{conf} = |A_i|^2 \sum_{a \in \text{FoV}}|A_{26}(\mathbf{\hat{n}}_a)T(\mathbf{\hat{n}}_a)|^2
    \label{eq:confusion}
\end{equation}
%\simon{I'm also confused by this: is there a secret $\delta(n_a-n_b)$ that was used?} \arcomment{Addressed now in the lead-up to this equation.}
So the confusion noise can be taken as the sum of the fluxes of the confusing sources (within the Galt telescope's field of view) weighted by the Galt beam response at their locations within the field of view, squared. 

To estimate this quantity, a point source sky was simulated in a HEALpix map (with $N_\text{side} = 256$) many (1000) times using the open-source radio sky simulation package \textit{cora} \footnote{\url{https://github.com/radiocosmology/cora/tree/master}}. The simulated point source sky has three ingredients: a Gaussian distributed background of dim sources below 0.1 Jy, a synthetic population drawn using the source count model of \citep{diMatteo} between 0.1 Jy and 10 Jy, and a catalog of real sources drawn from NVSS and VLSS above 10 Jy \citep{nvss, vlss}. These nominal flux thresholds are defined at 151 MHz and the latter 10 Jy threshold for real sources is scaled to the target frequency of the simulation. For each holography source, the sum in Equation \ref{eq:confusion} was then evaluated by summing over the squared beam-weighted fluxes of the sources taken within a ring centered on the location of the holography source and of diameter 2 times the FWHM of the Galt beam, using the beam model derived from the raster scan of Cas A described in Section \ref{sec:JG2D} and in \cite{galt_spie_proc}. We take the square root to obtain a quantity dimensionally compatible with the source flux, and we ignore the prefactor of the CHIME beam as there will be a compensating factor multiplying the source flux.  %\jm{Might be worth saying something like "The sum in Equation 9 was then evaluated \textit{for pointings centered on our primary holography targets} by summing..." When I first read the above statement, it wasn't clear that it was evaluated for our holography targets, but that said it certainly becomes clear in the next paragraph.}

The results of this procedure are summarized in Table \ref{tab:confusion} for 600\,MHz. For most holography sources - with the exceptions of 3C84, and 3C10C (which are near other real catalog sources) - the results are dominated by the random, synthetic background of sources, which are effectively spatially isotropic. For these holographic sources, over the ensemble of 1000 simulations, the confusion noise figure of Eq \ref{eq:confusion} has a median value under 1 Jy. As both the source flux and the confusion noise level are modulated by the CHIME beam in an actual measurement, in Table~\ref{tab:confusion} we present the average confusion noise figure as a percentage of the source flux at 600\,MHz. The reciprocal of this ratio represents the maximum ratio of signal to noise that is achievable with holography; e.g. in our worst case scenario using the very dim source 3C138 ($S_{600} \sim \SI{10}{Jy}$), the confusion noise level is about 10\% of the source flux, such that the peak achievable SNR we may expect is $\sim10$. 
%Ignoring the North-South modulation of the CHIME beam, the per-feed power beam of CHIME in the East-West direction typically drops to as much as $-20$ dB at the edges of the longest holography transits ($\sim \pm 30^\circ$ in hour angle). This suggests that for the brightest sources available to holography, we can avoid a confusion limit across the range of a typical holography transit. However, for the dimmer sources on the order of 10-30 Jy, the beam attenuation in the far sidelobes reduces the signal to be comparable to the confusion background at large hour angles, limiting the dynamic range of the holographic beam measurements at the declinations of these dimmer sources to the $\lesssim 10\%$ level. \tpm{But isn't the confusion noise equally attenuated by the CHIME beam response?}
 
\begin{deluxetable}{c c c c}
    \tablecaption{The 24 sources used for holography, their declinations, and their fluxes at 600 MHz, along with estimates for the holographic confusion noise (also at 600 MHz), expressed as a percentage of the source flux. These estimates are defined as in Eq \ref{eq:confusion}.  
    \label{tab:confusion}}
    \tablecolumns{4}
    \tablehead{
        \colhead{Source} & 
        \colhead{DEC [deg]} &
        \colhead{$S_{600}$ [Jy]} &
        \colhead{Conf. Noise [\%]}
    }
    \startdata
    Cyg A & 40.7 & 3613 & 0.02 \\ 
    Cas A & 58.8 & 2375 & 0.03 \\
    Tau A & 22.0 & 1142 & 0.06 \\
    Virgo A & 12.4 & 436 & .2 \\
    Hercules A & 5.0 & 120 & .6 \\
    3C353 & -1.0 & 106 & .7 \\
    Hydra A & -12.1 & 97 & .7 \\
    Perseus B & 29.7 & 87 & .8 \\ 
    3C10C & 64.2 & 71 & 7 \\
    3C273 & 2.1 & 55 & 1 \\
    3C84 & 41.5 & 38 & 10 \\
    3C295 & 52.2 & 37 & 2 \\
    3C58 & 64.8 & 31 & 2 \\
    3C161 & -5.9 & 30 & 2 \\
    3C147 & 49.9 & 29 & 2 \\
    3C111 & 38.0 & 29 & 2 \\
    3C196 & 48.2 & 28 & 2 \\
    3C409 & 23.6 & 27 & 3 \\
    3C358 & -21.5 & 26 & 3 \\
    3C48 & 33.2 & 25 & 3 \\
    3C286 & 30.5 & 18 & 4 \\
    3C454.3 & 16.1 & 12 & 6 \\
    3C78 & 4.1 & 11 & 6 \\
    3C138 & 16.6 & 10 & 7 \\
    \enddata
\end{deluxetable}

%{\subsubsection{\sout{CHIME gain Noise [Seth]}}}
%{\subsubsection{\sout{26m gain noise [Meiling]}}}
%{\subsubsection{\sout{Source variability (pulsars) [Tristan]}}}
%\lbn{I might recommend the instrumentation section go before the holography technique, and the confusion noise goes into the holography technique section. Probably I suggested something opposite before. I think you can remove the sout'd subsections at this point. \arcomment{Done!}}

